Dynamic Typography: Bringing Text to Life via Video Diffusion Prior

Text animation serves as an expressive medium, transforming static communication into dynamic experiences by infusing words with motion to evoke emotions, emphasize meanings, and construct compelling narratives. Crafting animations that are semantically aware poses significant challenges, demanding expertise in graphic design and animation. We present an automated text animation scheme, termed "Dynamic Typography", which combines two challenging tasks. It deforms letters to convey semantic meaning and infuses them with vibrant movements based on user prompts. Our technique harnesses vector graphics representations and an end-to-end optimization-based framework. This framework employs neural displacement fields to convert letters into base shapes and applies per-frame motion, encouraging coherence with the intended textual concept. Shape preservation techniques and perceptual loss regularization are employed to maintain legibility and structural integrity throughout the animation process. We demonstrate the generalizability of our approach across various text-to-video models and highlight the superiority of our end-to-end methodology over baseline methods, which might comprise separate tasks. Through quantitative and qualitative evaluations, we demonstrate the effectiveness of our framework in generating coherent text animations that faithfully interpret user prompts while maintaining readability. Our code is available at: https://animate-your-word.github.io/demo/.

==> sections/8.figure_only.tex <==

\begin{figure*}[!htb]
\centering
\includegraphics[width=1.0\textwidth]{pics/more_results.jpg}
\vspace{-0.5cm}
\caption{More Dynamic Typography results. Our generated animations vividly bring the specified letter to life while adhering to the prompt and maintaining legibility. Check our supplementary materials to see the full videos and more animations.}
\label{fig:more_results}
\end{figure*} 

% \begin{figure}[!ht]
% % \vspace{-0.2cm}
% \centering
% \includegraphics[width=1\columnwidth]{pics/ablation.jpg}
% \vspace{-0.5cm}
% \caption{Visual comparisons of ablation study. Some artifacts are highlighted in red cycles. Removing base shape or structure preservation regularization results in shape deviation and inconsistent artifacts. Without legibility regularization, each animation frame loses the letter ``R'' shape.}
% \label{fig:ablation}
% \end{figure} 

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=1\columnwidth]{pics/generalizability.jpg}
% \caption{Visual results of the same animation sample (``K'') using different text-to-video base models. All generated animations accurately depict the user's prompt and maintain the ``K'' shape, showing the generalizability of our methods across different text-to-video foundation models.}
% \label{fig:general}
% \end{figure} 

\begin{figure*}[!htb]
\centering
\includegraphics[width=1.0\textwidth]{pics/gen_fonts.jpg}
%\vspace{-0.5cm}
\caption{Dynamic Typography over different fonts for the same animation sample. The corresponding fonts in the first, second, and third rows are KaushanScript-Regular, Segoe Print, and Roboto-Bold respectively. The animated letter ``H'' preserves the unique style of each font while faithfully depicting the prompts, allowing it to be seamlessly integrated into the word ``HARMONY'' under different fonts.}
\label{fig:gen_fonts}
% \vspace{1cm}
\end{figure*} 

\begin{figure*}[!htb]
\centering
\includegraphics[width=1.0\textwidth]{pics/gen_prompts.jpg}
%\vspace{-0.5cm}
\caption{Dynamic Typography over different prompts for the same letter ``M'' to be animated. Our approach displays different visual effects based on three different prompts, offering a completely different reading experience for the same word.}
\label{fig:gen_prompts}
\end{figure*} 

\begin{figure*}[!htb]
\centering
\includegraphics[width=1.0\textwidth]{pics/gen_lan.jpg}
%\vspace{-0.5cm}
\caption{Dynamic Typography over different languages. In the first row, we animate the Chinese character ``从'' in the word ``跟从'', meaning ``following'' in English. In the second row, we animate the hiragana character 「つ」 from the Japanese word 「つり」, meaning ``fishing'' in English. This demonstrates the potential of our proposed methodology to generate Dynamic Typography over different languages.}
\label{fig:gen_lan}
\end{figure*} 
